Visualizing the Kinematics of Planet Formation

A stunning range of substructures in the dust of protoplanetary disks is routinely observed across a range of wavelengths. These gaps, rings and spirals are highly indicative of a population of unseen planets, hinting at the possibility of current observational facilities being able to capture planet-formation in action. Over the last decade, our understanding of the influence of a young planet on the dynamical structure of its parental disk has progressed significantly, revealing a host of potentially observable features which would betray the presence of a deeply embedded planet. In concert, recent observations have shown that subtle perturbations in the kinematic structure of protoplanetary disks are found in multiple sources, potentially the characteristic disturbances associated with embedded planets. In this work, we review the theoretical background of planet-disk interactions, focusing on the kinematical features, and the current methodologies used to observe these interactions in spatially and spectrally resolved observations. We discuss the potential pit falls of such kinematical detections of planets, providing best-practices for imaging and analysing interferometric data, along with a set of criteria to use as a benchmark for any claimed detection of embedded planets. We finish with a discussion on the current state of simulations in regard to planet-disk interactions, highlighting areas of particular interest and future directions which will provide the most significant impact in our search for embedded planets. This work is the culmination of the 'Visualizing the Kinematics of Planet Formation' workshop, held in October 2019 at the Center for Computational Astrophysics at the Flatiron Institute in New York City.

==> Visualizing the Kinematics of Planet Formation/theory_section.tex <==
% \subsubsection{MHD Zonal Flows}

% Magnetically induced zonal flows are considered to be one of the leading alternate mechanisms for ring formation.  Zonal flows are always axisymmetric and appear to be a robust outcome of numerical simulations that include magnetic fields, both without \cite[e.g.,][]{johansen2009, dzy2010, uribe2011, simon2012} and with \cite[e.g.,][]{lyra2008, simon2014, bai2014, bai2015, bethune2017, suriano2017, simon2018, Suriano_ea_2018, riols2019} a large scale vertical (i.e., oriented perpendicular to the disk plane) field threading the disk.

% The origin of flows with zero net field is still not well understood. Both local \citep{johansen2009,simon2012} and global \citep{dzy2010,uribe2011} simulations have been employed to characterize their properties, and have shown that the amplitude of the gas density variations can reach $\sim$ 20\% (though, see \citealt{dzy2010}, in which a $\sim$ 50\% variation was claimed). As for their lifetime, in local simulations (see \citealt{johansen2009}), these features do not necessarily last the entire duration of the simulation (which is, in general, considerably shorter than the age of protoplanetary disks), though this may depend on the domain size. \cite{dittrich2013} measure a typical lifetime of 50 local orbits for zonal flows.

% It has recently been demonstrated that in order to drive accretion at rates consistent with observations, a large-scale net vertical field must be present \citep{bai2013,simon2013a,simon2013b}. Thus, if MHD zonal flows are responsible for forming rings and gaps, there is a strong argument to be made that such zonal flows are of the net field variety.

% These net field zonal flows have appeared in both local \citep{bai2014,bai2015,simon2018,riols2019} and global \citep{lyra2008,bethune2017,suriano2017,Suriano_ea_2018,suriano2019,hu2019} simulations.
% %\footnote{We are ignoring global simulations that neglect the vertical component of stellar gravity.}
% These calculations have shown that the density variation (from gap to ring) is in general larger compared with zero net field simulations, but also span a large range in values.

% Another feature that emerges from these simulations is a larger concentration of magnetic flux within the gaps than within the rings. Broadly speaking, this suggests that a stronger outflow of gas would be present in the gap regions compared to the rings since a higher magnetic flux leads to a stronger wind \citep{simon2013b}. That this seems inconsistent with the results of \cite{Teague_ea_2019b}, in which an {\it inflow} into the gaps was observed from the kinematic data, is tempting as a way to rule out MHD zonal flows.  However, there remains much work to be done on the theory front.  For example, in the regions being probed by observations, will there still be a meridional flow present as suggested in \cite{Teague_ea_2019b}? This has not yet been ruled out by simulations.  Further analysis of these simulations is needed to determine the kinematic signatures of MHD zonal flows and how such signatures compare with current observations.

% \subsubsection{Viscous Instabilities}

% There have been a number of recent studies that have examined variants of a general process, known as the ``viscous instability".  In the language of classical $\alpha$ disk theory, this instability is present when $\partial{\rm ln}\alpha/\partial{\rm ln}\Sigma < 0$. In such a scenario, regions of lower surface density lead to an enhancement in accretion, creating an ``anti-diffusive" effect where regions that are over-dense become more so over time.

% If angular momentum transport in protoplanetary disks (and thus the disk viscosity) is set by the magnetorotational instability (MRI; \citealt{balbus1998})\footnote{The issue of whether or not the MRI is present in such disks, where the magnetic field may not be strongly coupled to the gas due to low ionization fractions, is currently a matter of strong debate.}, then one can cast this general viscous behavior within the context of such magnetically driven accretion by considering the layered accretion model \citep{gammie1996}. In this model, a low ionization mid-plane region is MRI-inactive (i.e., the dead zone), but is surrounded by layers that are MRI-active due to ionization from cosmic rays and stellar X-rays.


% This model led several groups \citep{wunsch2005,hasegawa2015} to propose a viscous-type instability. Given an increase in gas density at some radius, while the total column may increase, the column to which ionizing radiation penetrates (and thus the MRI active column) remains constant. Therefore, in a vertically averaged sense, the disk viscosity decreases as $\Sigma$ increases. A natural place for gas to pile up and thus initiate this instability is at the outer edge of the dead zone, beyond which the entire disk column is believed (at least until recently; see below) to become MRI-active again. Using one-dimensional models, \cite{hasegawa2015} demonstrated that indeed this region undergoes viscous instability, leading to sharp enhancements in the gas surface density.  However, the separation between the various ``gas bumps" was only $\sim 1$AU, and would be impossible to resolve with ALMA. Moreover, the 1D nature of the work cannot decide if the structures would produce rings or if they would break up azimuthally.

% In this regard, the Rossby wave instability (RWI; \citealt{lovelace1999}) stands as a robust process to break up rings into non-axisymmetric structures. The first work calculating the 2D hydrodynamical evolution of the dead/active zone boundary was presented by \cite{Varniere_Tagger2006}, in the context of the alpha viscosity model, showing breakdown into vortices by the RWI. These vortices concentrate dust grains and favor planet formation \citep{lyra2009,lyra2015}. As a rule of thumb, any ring that is narrowed than a scale height should break be unstable to the RWI. \cite{flock_2015} carried out full three-dimensional simulations of the same process, finding a well resolved ring/gap structure at the outer edge of the dead zone.  However, only one ring/gap pair was produced in their simulation, which disagrees with observations of many ringed systems where multiple rings/gaps are present \citep{Huang18}. Furthermore, as pointed out by \cite{ruge2016}, the rings of the \cite{flock_2015} simulations would likely undergo RWI and break into non-axisymmetric structure, as indeed shown by \cite{flock2017}.

% Finally, another variant of this instability, which included a more sophisticated treatment of dust physics, was studied in both a local \citep{johansen2011} and global \citep{dullemond2018} analysis.  While again, the presence of a viscous instability was indisputable, it is not clear that this instability is the origin of the observed rings.  In particular, \cite{dullemond2018} find that the strongest growing mode has a wavelength of the vertical gas scale height, suggesting that this is approximately the width of the pressure bumps that would arise from such an instability. This result is not particularly encouraging for this mechanism since the width of the observed gaps appear to range in size and are not necessarily equal to the gas scale height \citep{Huang18}.  However, it is worth noting that the \cite{johansen2011} simulation of the same process portrayed gas density variations larger than a scale height. Clearly, more work is required along this front.

% Ultimately, however, an uncertainty in all of these studies is the neglect of other low-ionization effects, known to be  relevant in protoplanetary disks: the Hall effect (see, e.g., \citealt{wardle1999,lesur2014,simon2015}) and ambipolar diffusion (see, e.g., \citealt{kunz2004, desch2004, bai2011, simon2013a, simon2013b}).  These additional effects complicate the notion of a sharp outer edge to the dead zone.  Further studies, both analytical and numerical, are required to address the presence of viscous instabilities within the context of this additional physics. If indeed such instabilities remain after including these effects, numerical simulations would then be needed to determine which kinematic signatures would emerge from the gaps and rings (or vortices) produced.


% \subsubsection{Secular Gravitational Instability}

% Protoplanetary disks contain about 2 percent solids, which, contrary to the gas, are not subject to a significant pressure force. Without pressure support hydrostatic equilibrium is not a possibility, so the solids are forced to accumulate in a denser sub-layer near the midplane of the disk. This enhances the solids-to-gas ratio in this region. Concurrently, the solids are loosely coupled to the gas via mutual drag forces. Although \citet{Goldreich_Ward1973} suggested direct gravitational collapse of solids in this sub-layer, they recognised the possible implications of the gas drag. With the inclusion of the gas drag on the solid phase, the Gravitational Instability of the solids turns into a drag-mediated, slow-acting (secular) instability, termed the secular gravitational instability \citep[sGI][]{Ward1976,ward2000}. This instability leads to inflow of additional solids into regions which already show a higher solid density than the surrounding disk on a shorter timescale than the decay timescale of the over-density, leading to the formation of multiple dust rings. In contrast to traditional GI, a dusty disk is always susceptible to secular GI, and collapse is only limited by the solid drift timescales and the disk lifetime. \citet{youdin2011} calculated the growth time of the instability including turbulent diffusion of solids due to gas-phase turbulence. He shows the growth rate to be on the order of $10^2$ yr in the most favourable case (low turbulence level, large grains, large orbital radii), although the growth rate increases significantly when smaller particles or higher turbulence levels are considered. The maximum turbulence level allowing secular GI is shown to be $\sim 10^{-3}$.

% The calculations for the traditional sGI only considered the equations for the solid phase and assumed the gas disk to be in steady state, not influenced by the dust. In reality however, the coupling of solid and gas phase acts both ways. \citet{takahashi2014} re-calculated the sGI using a full 2-fluid model. They show that a full treatment leads to more stringent conditions under which the sGI can grow, as the long wavelength modes previously thought unstable are stabilised by Coriolis forces. For their most favourable model, the growth time is $\sim 10^4$ yrs. The limit on gas turbulence is also lowered to $\alpha < 10^{-4}$. This does however not exclude sGI as a possible formation mechanism for the rings found in observations: \citet{Takahashi_Inutsuka_2016} show that the sGI is capalbe to form rings of $10$ AU width at disk radii outside 80 AU within $10^4$ yrs in conditions derived from HL Tau observations.

% %{\bf {\color{red} for Natascha to write}}

% \subsubsection{Infall-Induced Structures}

% %{\bf {\color{red} for Aleksandra to write}}
% \par Earlier phase objects still embedded within the protostellar envelope experience infall onto the disk, with infall rates of around $\dot{M} \sim 10^{-6}-10^{-5} \rm M_{\odot} \ yr^{-1}$ worth of material. This flux of mass and angular momentum no doubt has dynamical and structural consequences for the disk.
% \par Protostellar infall of envelope material can induce structure in the gas surface density profile creating pressure bumps by adding material to the disk, opening gaps due to the velocity shear of the landing material with respect to the disk, and triggering vortex formation through the RWI \citep{bae2015}. Perturbations in the pressure profile  have been shown to naturally concentrate dust into ring-like structures and protect mm-cm sized particles from radial drift \citep{pinilla2012}. \citet{bae2015} test several models of smooth protostellar infall in hydrodynamic simulations and find that cm sized dust grains are readily arranged into ring-like structures.
% \par Whether these structures could survive into the protoplanetary phase depends on the transport rate in those regions. Infalling material has the capability of generating large Reynold’s stresses; \citet{lesur2015} find that infall can induce spiral driven accretion with an effective $\alpha$ on the order of $10^{-2}$ in the outer disk. These large local transport rates have the potential to rapidly disrupt structures in the gas, without considering the triggering of other instabilities. In the absence of gaseous overdensities, long-term evolution of dust that may have been concentrated in these regions requires further study to determine observability of rings and gaps during the protoplanetary phase.
% While the oblique infall of material will have shear relative to the Keplerian velocity of the disk, the persistence of a kinematic structure in the absence of infalling material is unlikely.


% \subsubsection{Ice Line Related Structure}

% The composition of the solid component of protoplanetary disks changes almost discontinuously at the location of {\em ice lines}, at radii in the disk where the temperature matches the condensation temperature of specific chemical species. Ignoring for now the silicate ``ice" line---which is much too close-in to be resolved---abundance considerations imply that the water ice line (or snow line) is the most important \citep{Lodders03}. Other species of interest include ammonia and clathrates containing CO and N$_2$. The change in the condensable surface density across an ice line can lead directly to a radial variation in the opacity, which may be amplified by various indirect effects, including outward diffusion and re-condensation of vapor \citep{Stevenson88,Ros13} and sintering \citep{okuzumi16}. These processes modify the size distribution across the ice line, leading to changes in the radial drift speed and either particle pile-ups or deficits. Unlike many other physical processes that potentially generate rings, ice lines directly affect the {\em particle} distribution. Secondary gas-phase structure may nonetheless arise, for example due to feedback between the abundance of small grains and the efficiency of MHD-driven angular momentum transport processes \citep{Kretke07}.

% It is indisputable that ice lines ought to create axisymmetric structure in disks, but the size (and even sign) of the effect is hard to predict from first principles. Observationally, \citet{zhang2015} found that the ice lines of several major species aligned with the location of rings in HL~Tau, a result that they attributed to pebble growth near condensation fronts. The radii of rings in the DSHARP or Taurus samples, however, do not show the trend with stellar luminosity that would support the hypothesis that all rings are related to ice lines \citep{Huang18,Long2018}. Measuring the observable signatures of ice lines thus remains a largely open question, that would benefit from improved measurement of the mid-plane temperature profile.

% \subsubsection{Compositional Baroclinic Instability}

% Another possible way to produce rings in protoplanetary disks is the compositional baroclinic instability, identified by  \cite{loren-aguilar2015}. For small enough grains, the gas and the dust can be considered a single fluid, with lower pressure than a dust-free gas would have at the same density, since the grains do not produce pressure. As the grains settles, an entropy gradient develops between the settled dusty gas in the midplane, and the dust-poor gas in the upper layers. If the sedimentation is intense enough, this compositional entropy gradient eventually becomes superadiabatic, violating the Schwarzschild criterion for convection.

% Notice that the gas does not need to be non-isothermal. Even if the gas thermodynamics is isothermal, it is the dust-gas mixture that becomes baroclinic due to the entropy gradient established by the gradient of dust-to-gas ratio.

% \cite{loren-aguilar2015} derive the conditions for instability, finding

% \begin{equation}
% \left\vert\frac{\partial\varepsilon}{\partial z} \right\vert \gtrsim \frac{z}{h^2} \left(1+\varepsilon\right)\left[\gamma \frac{\partial\log\rho}{\partial\log p}-1+\frac{h^2}{z^2}\right]
% \end{equation}

% \noindent where $\varepsilon$ is the dust-to-gas ratio, $\gamma$ is the adiabatic index, $\rho$ is the density and $p$ is the pressure. The condition is valid for $\partial\varepsilon \partial z < 0$. For entropy gradients close to adiabatic the condition reduces to

% \begin{equation}
% \left\vert\frac{\partial\varepsilon}{\partial z} \right\vert \gtrsim  \frac{\left(1+\varepsilon\right)}{z}
% \end{equation}

% This condition is usually satisfied in the upper layers of disks, but becomes more difficult to sustain closer to the midplane. Small grains that are too well coupled do not lead to a strong enough compositional gradient to lead to instability; conversely, large enough solids will be too uncoupled and the single fluid approximation breaks down. The sweet spot depends depends on the friction time, which in turn is a function of the gas density, grain size and density.

% At saturation, the instability is characterized by toroidal vortices, with axisymmetric "vortex rolls" that gather dust into rings. The rings are narrow, with spacing of the order of $h_d$, the scale height of the dust layer. Since the dust scale height is smaller than the gas scale height, we can expect that these rings should not be resolved by ALMA at 10-50 AU, ruling it out as an explanation for most rings/gaps in disks observed to date.

% That still leaves the outer disk, at $\sim$100AU, as a possible location to observing the instability. Saturating in tens of local orbits, the instability could be observed at these locations within the disk lifetime.

% --- OLD SECTION 2 ---

% \cp{There is a bit of repetition with section 1.1 here. We should be able to cut a bit. I would be tempted to remove the first 2 paragraphs and add the few points that were not already mentioned in 1.1. The title of the section is also vitually the same as 1.1. I think we should only discuss kinematic detections here and update the title accordingly.}

% Detecting still-forming planets has the distinct problem that the planets are still embedded within their natal disk and thus surrounded by a non-negligible veil of material making direct detection exceptionally challenging. Indeed, most directly detected planets are in evolved systems where there is negligible contamination from the parental disk \citep[PDS~70 is a rare exception as the cavity in which the planets are detected is almost entirely void of gas and dust;][]{Keppler_ea_2019}. However, the interaction between an embedded planet and the surrounding gas and dust offers several observable features which can allow us to infer the presence of an otherwise unseen planet.

% The clearest of these is the carving of gaps and rings in the large grain distributions, resulting in distinct annular structure in both the NIR scattered light and mm~continuum, an overwhelmingly common feature in high-resolution observations of protoplanetary disks \citep{Andrews_ea_2018, DSHARP_II, Long_ea_2018}. Although rings in the dust structure have long been attributed to planet-opened gaps in the gas surface density \citep{Papaloizou_Lin_1984, Bryden_ea_1999, Nelson_ea_2000}, several other scenarios unrelated to embedded planets have been proposed and are able to reproduce the observations, such as magneto-rotational instabilities or zonal flows \citep[e.g.][]{flock_2015}. This degeneracy is because the dust reacts to the background gas density structure, accentuating regions of higher or lower density, but remaining agnostic about the underlying cause of the gas density perturbations. Although high spatial resolution observations may provide a way to distinguish between gap-opening mechanisms in the dust from differences in their radial morphology, contemporary observations limit such analyses to models assuming nested-Gaussians \citep[e.g.][]{dullemond2018b}.

==> theory_section.tex <==
% \subsubsection{MHD Zonal Flows}

% Magnetically induced zonal flows are considered to be one of the leading alternate mechanisms for ring formation.  Zonal flows are always axisymmetric and appear to be a robust outcome of numerical simulations that include magnetic fields, both without \cite[e.g.,][]{johansen2009, dzy2010, uribe2011, simon2012} and with \cite[e.g.,][]{lyra2008, simon2014, bai2014, bai2015, bethune2017, suriano2017, simon2018, Suriano_ea_2018, riols2019} a large scale vertical (i.e., oriented perpendicular to the disk plane) field threading the disk.

% The origin of flows with zero net field is still not well understood. Both local \citep{johansen2009,simon2012} and global \citep{dzy2010,uribe2011} simulations have been employed to characterize their properties, and have shown that the amplitude of the gas density variations can reach $\sim$ 20\% (though, see \citealt{dzy2010}, in which a $\sim$ 50\% variation was claimed). As for their lifetime, in local simulations (see \citealt{johansen2009}), these features do not necessarily last the entire duration of the simulation (which is, in general, considerably shorter than the age of protoplanetary disks), though this may depend on the domain size. \cite{dittrich2013} measure a typical lifetime of 50 local orbits for zonal flows.

% It has recently been demonstrated that in order to drive accretion at rates consistent with observations, a large-scale net vertical field must be present \citep{bai2013,simon2013a,simon2013b}. Thus, if MHD zonal flows are responsible for forming rings and gaps, there is a strong argument to be made that such zonal flows are of the net field variety.

% These net field zonal flows have appeared in both local \citep{bai2014,bai2015,simon2018,riols2019} and global \citep{lyra2008,bethune2017,suriano2017,Suriano_ea_2018,suriano2019,hu2019} simulations.
% %\footnote{We are ignoring global simulations that neglect the vertical component of stellar gravity.}
% These calculations have shown that the density variation (from gap to ring) is in general larger compared with zero net field simulations, but also span a large range in values.

% Another feature that emerges from these simulations is a larger concentration of magnetic flux within the gaps than within the rings. Broadly speaking, this suggests that a stronger outflow of gas would be present in the gap regions compared to the rings since a higher magnetic flux leads to a stronger wind \citep{simon2013b}. That this seems inconsistent with the results of \cite{Teague_ea_2019b}, in which an {\it inflow} into the gaps was observed from the kinematic data, is tempting as a way to rule out MHD zonal flows.  However, there remains much work to be done on the theory front.  For example, in the regions being probed by observations, will there still be a meridional flow present as suggested in \cite{Teague_ea_2019b}? This has not yet been ruled out by simulations.  Further analysis of these simulations is needed to determine the kinematic signatures of MHD zonal flows and how such signatures compare with current observations.

% \subsubsection{Viscous Instabilities}

% There have been a number of recent studies that have examined variants of a general process, known as the ``viscous instability".  In the language of classical $\alpha$ disk theory, this instability is present when $\partial{\rm ln}\alpha/\partial{\rm ln}\Sigma < 0$. In such a scenario, regions of lower surface density lead to an enhancement in accretion, creating an ``anti-diffusive" effect where regions that are over-dense become more so over time.

% If angular momentum transport in protoplanetary disks (and thus the disk viscosity) is set by the magnetorotational instability (MRI; \citealt{balbus1998})\footnote{The issue of whether or not the MRI is present in such disks, where the magnetic field may not be strongly coupled to the gas due to low ionization fractions, is currently a matter of strong debate.}, then one can cast this general viscous behavior within the context of such magnetically driven accretion by considering the layered accretion model \citep{gammie1996}. In this model, a low ionization mid-plane region is MRI-inactive (i.e., the dead zone), but is surrounded by layers that are MRI-active due to ionization from cosmic rays and stellar X-rays.


% This model led several groups \citep{wunsch2005,hasegawa2015} to propose a viscous-type instability. Given an increase in gas density at some radius, while the total column may increase, the column to which ionizing radiation penetrates (and thus the MRI active column) remains constant. Therefore, in a vertically averaged sense, the disk viscosity decreases as $\Sigma$ increases. A natural place for gas to pile up and thus initiate this instability is at the outer edge of the dead zone, beyond which the entire disk column is believed (at least until recently; see below) to become MRI-active again. Using one-dimensional models, \cite{hasegawa2015} demonstrated that indeed this region undergoes viscous instability, leading to sharp enhancements in the gas surface density.  However, the separation between the various ``gas bumps" was only $\sim 1$AU, and would be impossible to resolve with ALMA. Moreover, the 1D nature of the work cannot decide if the structures would produce rings or if they would break up azimuthally.

% In this regard, the Rossby wave instability (RWI; \citealt{lovelace1999}) stands as a robust process to break up rings into non-axisymmetric structures. The first work calculating the 2D hydrodynamical evolution of the dead/active zone boundary was presented by \cite{Varniere_Tagger2006}, in the context of the alpha viscosity model, showing breakdown into vortices by the RWI. These vortices concentrate dust grains and favor planet formation \citep{lyra2009,lyra2015}. As a rule of thumb, any ring that is narrowed than a scale height should break be unstable to the RWI. \cite{flock_2015} carried out full three-dimensional simulations of the same process, finding a well resolved ring/gap structure at the outer edge of the dead zone.  However, only one ring/gap pair was produced in their simulation, which disagrees with observations of many ringed systems where multiple rings/gaps are present \citep{Huang18}. Furthermore, as pointed out by \cite{ruge2016}, the rings of the \cite{flock_2015} simulations would likely undergo RWI and break into non-axisymmetric structure, as indeed shown by \cite{flock2017}.

% Finally, another variant of this instability, which included a more sophisticated treatment of dust physics, was studied in both a local \citep{johansen2011} and global \citep{dullemond2018} analysis.  While again, the presence of a viscous instability was indisputable, it is not clear that this instability is the origin of the observed rings.  In particular, \cite{dullemond2018} find that the strongest growing mode has a wavelength of the vertical gas scale height, suggesting that this is approximately the width of the pressure bumps that would arise from such an instability. This result is not particularly encouraging for this mechanism since the width of the observed gaps appear to range in size and are not necessarily equal to the gas scale height \citep{Huang18}.  However, it is worth noting that the \cite{johansen2011} simulation of the same process portrayed gas density variations larger than a scale height. Clearly, more work is required along this front.

% Ultimately, however, an uncertainty in all of these studies is the neglect of other low-ionization effects, known to be  relevant in protoplanetary disks: the Hall effect (see, e.g., \citealt{wardle1999,lesur2014,simon2015}) and ambipolar diffusion (see, e.g., \citealt{kunz2004, desch2004, bai2011, simon2013a, simon2013b}).  These additional effects complicate the notion of a sharp outer edge to the dead zone.  Further studies, both analytical and numerical, are required to address the presence of viscous instabilities within the context of this additional physics. If indeed such instabilities remain after including these effects, numerical simulations would then be needed to determine which kinematic signatures would emerge from the gaps and rings (or vortices) produced.


% \subsubsection{Secular Gravitational Instability}

% Protoplanetary disks contain about 2 percent solids, which, contrary to the gas, are not subject to a significant pressure force. Without pressure support hydrostatic equilibrium is not a possibility, so the solids are forced to accumulate in a denser sub-layer near the midplane of the disk. This enhances the solids-to-gas ratio in this region. Concurrently, the solids are loosely coupled to the gas via mutual drag forces. Although \citet{Goldreich_Ward1973} suggested direct gravitational collapse of solids in this sub-layer, they recognised the possible implications of the gas drag. With the inclusion of the gas drag on the solid phase, the Gravitational Instability of the solids turns into a drag-mediated, slow-acting (secular) instability, termed the secular gravitational instability \citep[sGI][]{Ward1976,ward2000}. This instability leads to inflow of additional solids into regions which already show a higher solid density than the surrounding disk on a shorter timescale than the decay timescale of the over-density, leading to the formation of multiple dust rings. In contrast to traditional GI, a dusty disk is always susceptible to secular GI, and collapse is only limited by the solid drift timescales and the disk lifetime. \citet{youdin2011} calculated the growth time of the instability including turbulent diffusion of solids due to gas-phase turbulence. He shows the growth rate to be on the order of $10^2$ yr in the most favourable case (low turbulence level, large grains, large orbital radii), although the growth rate increases significantly when smaller particles or higher turbulence levels are considered. The maximum turbulence level allowing secular GI is shown to be $\sim 10^{-3}$.

% The calculations for the traditional sGI only considered the equations for the solid phase and assumed the gas disk to be in steady state, not influenced by the dust. In reality however, the coupling of solid and gas phase acts both ways. \citet{takahashi2014} re-calculated the sGI using a full 2-fluid model. They show that a full treatment leads to more stringent conditions under which the sGI can grow, as the long wavelength modes previously thought unstable are stabilised by Coriolis forces. For their most favourable model, the growth time is $\sim 10^4$ yrs. The limit on gas turbulence is also lowered to $\alpha < 10^{-4}$. This does however not exclude sGI as a possible formation mechanism for the rings found in observations: \citet{Takahashi_Inutsuka_2016} show that the sGI is capalbe to form rings of $10$ AU width at disk radii outside 80 AU within $10^4$ yrs in conditions derived from HL Tau observations.

% %{\bf {\color{red} for Natascha to write}}

% \subsubsection{Infall-Induced Structures}

% %{\bf {\color{red} for Aleksandra to write}}
% \par Earlier phase objects still embedded within the protostellar envelope experience infall onto the disk, with infall rates of around $\dot{M} \sim 10^{-6}-10^{-5} \rm M_{\odot} \ yr^{-1}$ worth of material. This flux of mass and angular momentum no doubt has dynamical and structural consequences for the disk.
% \par Protostellar infall of envelope material can induce structure in the gas surface density profile creating pressure bumps by adding material to the disk, opening gaps due to the velocity shear of the landing material with respect to the disk, and triggering vortex formation through the RWI \citep{bae2015}. Perturbations in the pressure profile  have been shown to naturally concentrate dust into ring-like structures and protect mm-cm sized particles from radial drift \citep{pinilla2012}. \citet{bae2015} test several models of smooth protostellar infall in hydrodynamic simulations and find that cm sized dust grains are readily arranged into ring-like structures.
% \par Whether these structures could survive into the protoplanetary phase depends on the transport rate in those regions. Infalling material has the capability of generating large Reynold’s stresses; \citet{lesur2015} find that infall can induce spiral driven accretion with an effective $\alpha$ on the order of $10^{-2}$ in the outer disk. These large local transport rates have the potential to rapidly disrupt structures in the gas, without considering the triggering of other instabilities. In the absence of gaseous overdensities, long-term evolution of dust that may have been concentrated in these regions requires further study to determine observability of rings and gaps during the protoplanetary phase.
% While the oblique infall of material will have shear relative to the Keplerian velocity of the disk, the persistence of a kinematic structure in the absence of infalling material is unlikely.


% \subsubsection{Ice Line Related Structure}

% The composition of the solid component of protoplanetary disks changes almost discontinuously at the location of {\em ice lines}, at radii in the disk where the temperature matches the condensation temperature of specific chemical species. Ignoring for now the silicate ``ice" line---which is much too close-in to be resolved---abundance considerations imply that the water ice line (or snow line) is the most important \citep{Lodders03}. Other species of interest include ammonia and clathrates containing CO and N$_2$. The change in the condensable surface density across an ice line can lead directly to a radial variation in the opacity, which may be amplified by various indirect effects, including outward diffusion and re-condensation of vapor \citep{Stevenson88,Ros13} and sintering \citep{okuzumi16}. These processes modify the size distribution across the ice line, leading to changes in the radial drift speed and either particle pile-ups or deficits. Unlike many other physical processes that potentially generate rings, ice lines directly affect the {\em particle} distribution. Secondary gas-phase structure may nonetheless arise, for example due to feedback between the abundance of small grains and the efficiency of MHD-driven angular momentum transport processes \citep{Kretke07}.

% It is indisputable that ice lines ought to create axisymmetric structure in disks, but the size (and even sign) of the effect is hard to predict from first principles. Observationally, \citet{zhang2015} found that the ice lines of several major species aligned with the location of rings in HL~Tau, a result that they attributed to pebble growth near condensation fronts. The radii of rings in the DSHARP or Taurus samples, however, do not show the trend with stellar luminosity that would support the hypothesis that all rings are related to ice lines \citep{Huang18,Long2018}. Measuring the observable signatures of ice lines thus remains a largely open question, that would benefit from improved measurement of the mid-plane temperature profile.

% \subsubsection{Compositional Baroclinic Instability}

% Another possible way to produce rings in protoplanetary disks is the compositional baroclinic instability, identified by  \cite{loren-aguilar2015}. For small enough grains, the gas and the dust can be considered a single fluid, with lower pressure than a dust-free gas would have at the same density, since the grains do not produce pressure. As the grains settles, an entropy gradient develops between the settled dusty gas in the midplane, and the dust-poor gas in the upper layers. If the sedimentation is intense enough, this compositional entropy gradient eventually becomes superadiabatic, violating the Schwarzschild criterion for convection.

% Notice that the gas does not need to be non-isothermal. Even if the gas thermodynamics is isothermal, it is the dust-gas mixture that becomes baroclinic due to the entropy gradient established by the gradient of dust-to-gas ratio.

% \cite{loren-aguilar2015} derive the conditions for instability, finding

% \begin{equation}
% \left\vert\frac{\partial\varepsilon}{\partial z} \right\vert \gtrsim \frac{z}{h^2} \left(1+\varepsilon\right)\left[\gamma \frac{\partial\log\rho}{\partial\log p}-1+\frac{h^2}{z^2}\right]
% \end{equation}

% \noindent where $\varepsilon$ is the dust-to-gas ratio, $\gamma$ is the adiabatic index, $\rho$ is the density and $p$ is the pressure. The condition is valid for $\partial\varepsilon \partial z < 0$. For entropy gradients close to adiabatic the condition reduces to

% \begin{equation}
% \left\vert\frac{\partial\varepsilon}{\partial z} \right\vert \gtrsim  \frac{\left(1+\varepsilon\right)}{z}
% \end{equation}

% This condition is usually satisfied in the upper layers of disks, but becomes more difficult to sustain closer to the midplane. Small grains that are too well coupled do not lead to a strong enough compositional gradient to lead to instability; conversely, large enough solids will be too uncoupled and the single fluid approximation breaks down. The sweet spot depends depends on the friction time, which in turn is a function of the gas density, grain size and density.

% At saturation, the instability is characterized by toroidal vortices, with axisymmetric "vortex rolls" that gather dust into rings. The rings are narrow, with spacing of the order of $h_d$, the scale height of the dust layer. Since the dust scale height is smaller than the gas scale height, we can expect that these rings should not be resolved by ALMA at 10-50 AU, ruling it out as an explanation for most rings/gaps in disks observed to date.

% That still leaves the outer disk, at $\sim$100AU, as a possible location to observing the instability. Saturating in tens of local orbits, the instability could be observed at these locations within the disk lifetime.

% --- OLD SECTION 2 ---

% \cp{There is a bit of repetition with section 1.1 here. We should be able to cut a bit. I would be tempted to remove the first 2 paragraphs and add the few points that were not already mentioned in 1.1. The title of the section is also vitually the same as 1.1. I think we should only discuss kinematic detections here and update the title accordingly.}

% Detecting still-forming planets has the distinct problem that the planets are still embedded within their natal disk and thus surrounded by a non-negligible veil of material making direct detection exceptionally challenging. Indeed, most directly detected planets are in evolved systems where there is negligible contamination from the parental disk \citep[PDS~70 is a rare exception as the cavity in which the planets are detected is almost entirely void of gas and dust;][]{Keppler_ea_2019}. However, the interaction between an embedded planet and the surrounding gas and dust offers several observable features which can allow us to infer the presence of an otherwise unseen planet.

% The clearest of these is the carving of gaps and rings in the large grain distributions, resulting in distinct annular structure in both the NIR scattered light and mm~continuum, an overwhelmingly common feature in high-resolution observations of protoplanetary disks \citep{Andrews_ea_2018, DSHARP_II, Long_ea_2018}. Although rings in the dust structure have long been attributed to planet-opened gaps in the gas surface density \citep{Papaloizou_Lin_1984, Bryden_ea_1999, Nelson_ea_2000}, several other scenarios unrelated to embedded planets have been proposed and are able to reproduce the observations, such as magneto-rotational instabilities or zonal flows \citep[e.g.][]{flock_2015}. This degeneracy is because the dust reacts to the background gas density structure, accentuating regions of higher or lower density, but remaining agnostic about the underlying cause of the gas density perturbations. Although high spatial resolution observations may provide a way to distinguish between gap-opening mechanisms in the dust from differences in their radial morphology, contemporary observations limit such analyses to models assuming nested-Gaussians \citep[e.g.][]{dullemond2018b}.
